AutoPSV: Automated Process-Supervised Verifier

In this work, we propose a novel method named \textbf{Auto}mated \textbf{P}rocess-\textbf{S}upervised \textbf{V}erifier (\textbf{\textsc{AutoPSV}}) to enhance the reasoning capabilities of large language models (LLMs) by automatically annotating the reasoning steps. \textsc{AutoPSV} begins by training a verification model on the correctness of final answers, enabling it to generate automatic process annotations. This verification model assigns a confidence score to each reasoning step, indicating the probability of arriving at the correct final answer from that point onward. We detect relative changes in the verification's confidence scores across reasoning steps to automatically annotate the reasoning process, enabling error detection even in scenarios where ground truth answers are unavailable. This alleviates the need for numerous manual annotations or the high computational costs associated with model-induced annotation approaches. We experimentally validate that the step-level confidence changes learned by the verification model trained on the final answer correctness can effectively identify errors in the reasoning steps. We demonstrate that the verification model, when trained on process annotations generated by \textsc{AutoPSV}, exhibits improved performance in selecting correct answers from multiple LLM-generated outputs. Notably, we achieve substantial improvements across five datasets in mathematics and commonsense reasoning. The source code of \textsc{AutoPSV} is available at \url{https://github.com/rookie-joe/AutoPSV}.

==> sections/checklist.tex <==

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  The main claims made in the ``abstract'' and ``introduction'' sections accurately reflect the paper's contributions and scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the limitations in the ``Limitations'' section attached in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper focuses on exploring a novel process-supervision approach to enhance verifiers, and as such, it is primarily based on experimental results rather than theoretical proofs. The paper does not introduce new theoretical results; instead, it relies on theorems that have already been proven in previously published literature. These referenced theorems are clearly cited in the ``Method'' section of the paper, indicating that the authors have not provided new proofs but have utilized established results to support their experimental work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper includes all the necessary information required to reproduce the main experimental results. This information is detailed within the ``Experiment'' section and the ``Appendix'' of the paper, ensuring that readers have access to the methodologies, parameters, and data needed to validate the main claims and conclusions presented.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the training scripts in the supplementary material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides comprehensive details regarding the training and testing in the ``Appendix'' due to the page limit.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We mentioned in ``Experiment'' section that \textit{The results are presented with an accuracy of ±0.1, calculated at a 95\% confidence level}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include sufficient information regarding the computer resources required to reproduce the experiments in ``Experiment'' and ``Appendix''. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the societal impact of the work in the ``Broader Impact'' section attached in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not present any high-risk data or models that could be prone to misuse, as it is focused on enhancing the performance of Language Model Support Systems (LLMS) within the field of Natural Language Processing (NLP).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, all experiments conducted in the paper utilize open-source models. Proper references and citations are included in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the code in the supplementary materials and include a README file with details about data annotation, training, and limitations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}




==> sections/experiment-no-comment.tex <==
\section{Experiment}


\subsection{Experiment on Selective Model Performance}
\label{sec:gsm8k_selection_result}
In our experiment, we fine-tuned the Mistral-7B model using training data generated by sampling the Mistral model on GSM8K training prompts 100 times. Each sample was annotated with ground truth labels to indicate correctness. This process resulted in the creation of a selective model. For the evaluation phase, we utilized the Mistral-7B, Mixtral 8 $\times$ 7B, and Qianwen-70B models, sampling each 5 times. The selective model, trained from Mistral, was then applied to choose the best output, denoted as SIE. This method was benchmarked against self-consistency (SC), with the understanding that the upper limit of these methods is the accuracy of the model's pass5. The experimental results are summarized in the table below:


\begin{table}[ht]
\centering
\caption{Experimental results showing the performance of selective models across different configurations.}
\label{tab:table1}
\begin{tabular}{lcccccc}
\toprule
Model      & Pass@1 & Pass@5 & SC    & SIE, Mistral & SIE, Phi & SIE, Gemma \\
\midrule
Mistral-Instruct    & 42.08                 & 69.90 & 50.03 & 60.72                         & 52.61    & 40.56      \\
Mixtral-Instruct  & 62.55       & 82.31 & 69.06 & 74.07                         & 69.37    & 52.92      \\
Qwen & 77.03             & 91.13 & 81.27 & 85.00                         & 84.19    & 74.45      \\
\bottomrule
\end{tabular}
\end{table}



The results demonstrate the effectiveness of the selective model, particularly when applied to the ensemble and larger Qianwen-70B models, resulting in significant performance improvements across all metrics compared to baseline one-sample and pass5 accuracies. Notably, the selective model (SIE), trained from Mistral, shows a substantial increase in accuracy, validating the potential of our approach for enhancing model selection strategies.


\paragraph{Performance Analysis of Different Selectors}
The performance disparity among the selectors can be attributed primarily to variations in model sizes and the accuracy of their training data. Table \ref{tab:model_data} presents a consolidated view of the model sizes along with the accuracy metrics of their training data.

\begin{table}[ht]
\centering
\caption{Model sizes and training data accuracy for different selectors.}
\label{tab:model_data}
\begin{tabular}{lccccc}
\toprule
Model      & Model Size & Training Data Pass@100 \\
\midrule
Mistral    & 7B         & 0.9914                           \\
Phi-2      & 2B         & 0.9605                            \\
Gemma   & 2B         & 0.8971                        \\
\bottomrule
\end{tabular}
\end{table}


As shown in Table \ref{tab:model_data}, the Mistral model, being the largest at 7B parameters, demonstrates superior performance. This is likely due to its increased capacity for complex pattern recognition and decision-making. In contrast, both Phi-2 and Gemma-2B are 2B models, yet they show varied performance metrics. This variance can be further explained by the quality of their training data. For instance, Phi-2's training data has higher Pass@100 and SC (Self Consistency) scores compared to Gemma-2B, which is reflected in its better performance in the experimental results shown in Table \ref{tab:table1}.

In summary, the performance differences among the selectors are influenced by both the inherent capacity of the models, dictated by their size and the quality of their training data, highlighting the importance of both aspects in developing effective machine learning models.




\subsection{Detecting Hallucination During Math Reasoning}
\label{sec:pch}
By predicting the likelihood of future correctness as shown in~Eq.\eqref{eq:mse-loss}, we explore our models' potential to detect procedural errors. 
In Section \Cref{sec:pch-definition}, we delineate our definition of \textit{Process Calculation Hallucination} and establish a preliminary benchmark. 
Subsequently, in~\Cref{sec:pch-detection}, we elaborate on how to utilize the trained model for procedural detection and evaluate this approach against the benchmark outlined in~\Cref{sec:pch-definition}.
\subsubsection{Process Calculation Hallucination}
\label{sec:pch-definition}
We delineate a ground truth creation process for labeling \textit{process calculation hallucination}~(PCH). 
We define \textit{process calculation hallucination} as the phenomenon where, within a computational expression, the numerical values on either side of the equals sign do not match. 
This discrepancy signifies a failure in the computational reasoning process, marking the specific instance as hallucinatory within the context of mathematical calculations.


\begin{table}[ht]
\centering
\caption{Results of LlaMA2 model on GSM8K training data via few-shot cot prompting for five sampling iterations.}
\label{tab:llama2chat_results}
\begin{tabular}{lccc}
\toprule
Model         & Pass@5 & Self Consistency  & PCH \\
\midrule
LlaMA2     & 0.4791 & 0.2881 & 0.1824\\
\bottomrule
\end{tabular}
\end{table}

In our methodology, LlaMA2 is prompted to delineate the calculation process within specific markers (\texttt{<< >>}). Using regular expressions, we extract the content within these markers. The extracted expressions, positioned left of the "=" sign, are evaluated through Python's `eval` function to ascertain their equivalence with the right-hand side results.

Instances lacking markers (\texttt{<< >>}) or containing unevaluable expressions due to unsolvability or incorrect formatting (e.g., "x + 1 + 2 = 4") are classified as non-calculative and omitted from the ground truth labels. This stratagem ensures that our ground truth accurately mirrors the model's computational inaccuracies during reasoning, thereby preventing any overestimation of computational accuracy.

Notably, while entities like DeepMind have engaged in similar annotation efforts with numerous human labelers, categorizing them as "trace errors," our methodology leverages Python's `eval` function for automatic labeling. This approach offers scalability and an efficient means of reflecting trace errors to some extent.


\subsubsection{Process Calculation Hallucination Detection}
\label{sec:pch-detection}
To detect hallucinations during the process of math reasoning, we utilize the scoring mechanism provided by the SIE models. Instead of solely evaluating the final output, we assess the confidence change between intermediate steps of the reasoning process.

We define the confidence change as:
\begin{align}
   \label{eq:relative-confidence-change}
    \begin{aligned}
       \frac{{f_{\bm{\theta}}(q; S^{(1:t + T)}) - f_{\bm{\theta}}(q; S^{(1:t)})}}{{f_{\bm{\theta}}(q; S^{(1:t)})}}
    \end{aligned}
\end{align}
where \(f_{\bm{\theta}}(q; S^{(1:t)})\) represents the model's confidence score at step \(t\) and \(f_{\bm{\theta}}(q; S^{(1:t + T)})\) represents the confidence score at step \(t+T\). A negative relative change indicates a decrease in confidence.

To illustrate this process, consider the following example:

\begin{tcolorbox}
\textbf{Question:} Randy just turned 12 and started playing the piano. His friend Sheila told him about the 10,000-hour rule which says, after 10,000 hours of practice, you become an expert or master in your field. If Randy wants to become a piano expert before he is 20, how many hours a day will he need to practice if he practices every day, Monday – Friday, and takes two weeks off for vacation each year?

\textbf{Solution:}
\begin{enumerate}
    \item If Randy wants to become a piano expert before he is 20, he will need to practice for 10,000 hours in total. Since he is 12 now, that means he will need to practice for \(10,000/20 = 500\) hours a year.
    \item \textcolor{red}{\texttt{<Error>}} If he practices every day, Monday – Friday, that means he will need to practice for 500*52 = \texttt{<<}500*52=\textcolor{red}{260}\texttt{>>} 260 weeks.  \textcolor{red}{\texttt{<Error>}}
    \item  Since he takes two weeks off for vacation each year, that means he will need to practice for \(260/52 = 5\) hours a day. 
    \item The answer is 5.
\end{enumerate}
\end{tcolorbox}

In this instance, the highlighted errors in red signify hallucinations during the reasoning process. This is detected by the model's confidence decreasing significantly.




\subsubsection{Quantitative Results}
\Cref{tab:pch_detection_results} presents the performance metrics for Process Calculation Hallucination Detection, showcasing an accuracy of 0.8504, a recall of 0.9029, and an F1-score of 0.8759. The high recall indicates that the model is proficient at identifying most of the true positive cases, i.e., it effectively detects when hallucinations occur in the reasoning process. The accuracy, slightly lower than the recall, suggests that the model also performs well in correctly labeling both hallucinatory and non-hallucinatory instances. The F1-score, which balances precision and recall, stands at 0.8759, demonstrating a strong overall performance of the model in detecting hallucinations during mathematical reasoning. This indicates that the model is not only good at detecting the presence of hallucinations (as evidenced by high recall) but also at maintaining a balanced detection rate (as evidenced by the F1-score).
\begin{table}[ht]
\centering
\caption{Performance metrics for Process Calculation Hallucination Detection}
\label{tab:pch_detection_results}
\begin{tabular}{lccc}
\toprule
Metric & Accuracy & Recall & F1-Score \\
\midrule
Value  & 0.8504   & 0.9029 & 0.8759   \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Self-Evolution for Selector Improvement}
This section describes a methodological shift from relying on sparse, ground-truth-based outcome labels to adopting nuanced, self-generated process labels for process supervision.

\subsubsection{Self-Evolution Loss}
Originally, the loss function (Eq.~\eqref{eq:mse-loss}) utilized \(y^i\), a sparse label representing the binary correctness of the final answer compared to the ground truth. This label remained \textbf{constant} across all solution steps:
\begin{align*}
    \begin{aligned}  
         l_{\text{Original}}(q; S_i^{(1:t)}, y^i) = \left(f_{\bm{\theta}}(q; S_i^{(1:t)}) - y^i\right)^2.
    \end{aligned}
\end{align*}
To provide a more nuanced understanding, we introduce a revised loss function where \(y^{i,t}\) dynamically reflects correctness at each solution step:
\begin{align}
\label{eq:mse-loss-process-supervision}
    \begin{aligned}  
         l_{\text{SELF}}(q; S_i^{(1:t)}, y^{i,t}) = \left(f_{\bm{\theta}}(q; S_i^{(1:t)}) - y^{i,t}\right)^2.
    \end{aligned}
\end{align}
\(y^{i,t}\) is determined by a detection method detailed in~\Cref{sec:pch-detection}, which evaluates the change in the model's confidence over solution steps.
Specifically, we compare the relative change defined as Eq.~\eqref{eq:relative-confidence-change} against a predefined threshold \(\theta\). If the change exceeds \(\theta\), it indicates a significant negative shift, prompting an adjustment of the label from 1 to 0.\footnote{We note that once an error is identified at \(t^{th}\) step, all subsequent \(y^{i,t' | t' \geq t}\) is labeled as 0. This labeling strategy termed the "locate the first error process," ensures that any detected error influences the labeling of all following steps (todo: add a citation of the same labeling strategy from deepmind).}



\subsubsection{Experiments}
We present two experimental results to demonstrate the efficacy of our proposed approach. 

\textbf{Outcome-Supervised(OS) vs. Process-Supervised (PS) training.} We utilize an outcome-supervised trained model to relabel the process-supervised training data, adhering to Eq. \eqref{eq:mse-loss-process-supervision}. We then retrain a new model using this relabeled data. This experiment highlights the performance gap between outcome-supervised and process-supervised training.



\begin{table}[ht]
\centering
\caption{Comparison of outcome-supervised (OS) and process-supervised (PS) training performance for different Selected Candidates.}
\label{tab:outcome-supervised-vs-process-supervised-training}
\begin{tabular}{lcc}
\toprule
Selected Candidates & OS &  PS \\
\midrule
Mistral-Instruct & 60.72 & 59.14 \\
Mixtral-Instruct & 74.07 & 68.39\\
Qwen-72b & 84.19 & 83.70 \\
\bottomrule
\end{tabular}
\end{table}

We note that our process-supervised model was trained using data from the output-supervised model. The small performance gap between the process-supervised and output-supervised models shows that the relabeled process-supervised training method successfully inherits information from the outcome-supervised model without requiring ground truth annotations. This finding provides a fundamental guarantee for our subsequent self-evolution approach.

\textbf{Continuous Self-Evolution.} We further leverage the process-labeling strategy to empower the model to autonomously annotate prompts for continuous self-evolution starting from the outcome-supervised trained model, freeing it from the constraints of human labeling.
\begin{table}[ht]
\centering
\caption{Evaluation of Models on GSM8K and Math Benchmarks}
\label{tab:self_evolution_evaluation_math}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{GSM8K} & \multicolumn{2}{c}{MATH} & \multicolumn{2}{c}{Mistral-SIE} & \multicolumn{2}{c}{Mistral-SIE-SELF}  \\
                       & Pass@5 & Self-Cons. & Pass@5 & Self-Cons. &   GSM8K & MATH   &   GSM8K & MATH                \\
\midrule
Mistral-Instruct       & 69.90  & 50.03      & 7.7   & 1.64       & 61.18 & 5.10    & &           \\
Mixtral-Instruct       & 82.30  & 69.06      & 22.80  & 10.66      & 74.91 & 15.2       & &          \\
Qwen-72b               & 91.13  & 81.27      & 56.10  & 40.10      & 84.91 & 38.94      & &          \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[ht]
\centering
\caption{Evaluation of Models on Reasoning Benchmarks}
\label{tab:self_evolution_evaluation_reason}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{HellaSwag} & \multicolumn{2}{c}{Winogrande} &  \multicolumn{2}{c}{Anli}  & \multicolumn{2}{c}{Mistral-SIE} & \multicolumn{2}{c}{Mistral-SIE-SELF}  \\
                       & Pass@5 & Self-Cons. & Pass@5 & Self-Cons. &  Pass@5 & Self-Cons. &  &&&               \\
\midrule
Mistral-Instruct      & 76.84  & 40.30  &   91.16 &   58.64   & 73.4 &     45.6      \\
Mixtral-Instruct       & 84.05  &  73.67 & 79.16  &   68.75      & 68.4 &   59.0  \\
Qwen-72b               & 95.28  &  85.44 & 88.63  &   72.21     & 82.4 &  63.8  \\
\bottomrule
\end{tabular}
}
\end{table}

In our evaluation process, we present language models with a set of few-shot in-context examples along with corresponding questions. We follow the standard evaluation methodology outlined in~\cite{eval-harness}, employing the ``Accuracy'' metric to ensure consistency across all benchmarks.
For more reliable pass@k results, we adopt the calculation approach specified in~\cite{humaneval}. Specifically, we generate 20 samples per task, assessing the number of correct samples that pass unit tests, and then calculating the unbiased estimator for pass@k. 
To obtain the self-consistency and SIE results, we randomly select 5 over 20 samples and perform the calculations separately.
The results are accurate up to ±0.01 for a 95\% confidence level.
For additional implementation details, please refer to \Cref{app:experiment_details}.














==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}


Large language models (LLMs) have demonstrated remarkable capabilities across various tasks~\citep{gpt35turbo,GPT4,mistrallarge,claude3}. Nonetheless, even the state-of-the-art LLMs still face challenges in their reasoning abilities,\ZY{~e.g., the can only achieve .} \ZYQ{Agree with Jamie, another choice is to simply report their number.} This includes complex multi-step mathematical reasoning that involves computations~\citep{Arkoudas2023Corr,VerifyStep2023,Huang2023Corr,Zicheng2024Corr} and commonsense reasoning that requires an understanding of contextual relationships and logical inferences~\citep{Arkoudas2023Corr,Hanmeng2023Corr,Liangming2023EMNLP,Boshi2023EMNLP,Ruixin2023ACL}.

Previous research has explored various approaches to address these challenges. One approach involves model training or instruction tuning using a substantial amount of chain-of-thought (CoT) reasoning data~\citep{Chung2022,Mukherjee2023,Gunasekar2023,Luo2023}, which aims to improve the model's ability to generate step-by-step reasoning. Another approach is prompting~\citep{CoT,ComplexityCoT}, where the model is provided with specific prompts or instructions to encourage it to generate intermediate reasoning steps. This can be done through few-shot prompting with augmented demonstration exemplars that include intermediate steps~\citep{gpt3,CoT,ComplexityCoT}, or zero-shot prompting with specific instructions that explicitly ask the model to show certain intermediate steps~\citep{KojimaGRMI22,Analogical}. Additionally, verification techniques~\citep{ProcessFeedback2022,StepAware2023,VerifyStep2023} have been explored, where a separate verification model is trained to evaluate and potentially correct the reasoning process generated by a large language model.  
Among these techniques, verification has  have gained attention. \ZYQ{may be we can remove this sentence? "Among these techniques, verification has  have gained attention.".}
The motivation behind verification is that LLMs may not always output the correct answer with the highest confidence score. \ZYQ{ this sentence is not clear. "may not always output the correct answer with the highest confidence score" is there any evidence?}
Additionally, training a separate verification model can be much more efficient than directly optimizing or prompting the original large model, as the verification model can be significantly smaller in size~\citep{Scheurer2023Corr}. 
% In other words, the correct answer could exist within the model's broader exploration space across multiple samples, rather than solely in its greedily selected output. 
% verification models can rerank the outputs, potentially achieving higher accuracy by considering a wider exploration of the reasoning problem.
\ZYQ{I think the above paragraph is too long. Too much introduction of the existing methods will weaken the technical contribution of our paper.}

Verification models generally fall into two training paradigms: outcome supervision and process supervision. In outcome supervision, the training annotations rely on the correctness of the final answer~\citep{CobbeGSM8k2021, YuOVM2023}, while in process supervision, the annotations are based on evaluations of each reasoning step~\citep{RewardStep2023,VerifyStep2023,StepAware2023}. \ZY{Process supervision is demanding in terms of annotations. Typically, it relies on either expensive and highly skilled human evaluators~\citep{RewardStep2023,VerifyStep2023} or model-induced process annotations~\citep{MiPS2024,MathShepherd2023} to estimate the future correctness of the current reasoning step using Monte Carlo tree search~\citep{Coulom06,SilverHMGSDSAPL16}. In contrast, outcome supervision only requires annotations for the output, making it more economical in terms of annotation effort but less effective. That being said, when questions answering involved multiple reasoning paths, all aforementioned model-induced methods requires numerous samples to ensure accurate estimations.} 

\ZYQ{I feel like we need to promote our method a little more.}
\ZY{In this paper, we present a novel method named Automated Process Labeling via Confidence Variation (\name), which enjoys the both advantages of process supervision and output supervision. Our method starts from utilizing outcome supervision annotations to learn an outcome-supervised verification model. Then, this model assigns step-level scores to unannotated intermediate reasoning steps, which estimated the confidence in each reasoning step's likelihood of leading to a correct final answer.  By calculating the relative confidence variation, we could produce process annotations with significantly reduced effort for annotating. With our process supervision data, we train a LLM model, resulting in a process-supervised enhanced verification model. The overall framework of our method is illustrated in~\Cref{fig:orm_process_annotation}.


We conduct extensive experiments across five datasets, including mathematical reasoning benchmarks and commonsense reasoning tasks. The results demonstrate that our method effectively improves the reasoning capability of the model with our highly efficient labeling scheme for process supervision, killing two birds with one stone.

In summary, our contribution is as follows:
\begin{itemize}
\vspace{-1mm}
\item We introduce AUTOCV, a method for automatically labeling process data to enhance the reasoning capabilities of large language models (LLMs). Our approach combines the strengths of output supervision and process supervision to automatically annotate reasoning steps.
\item AUTOCV effectively identifies variations in model confidenhe cce to annotate torrectness of intermediate reasoning steps, enabling efficient automatic labeling for process supervision.
\item Comprehensive experiments demonstrate that process supervision data generated by AUTOCV significantly improves the performance and scalability of verification models in mathematical and commonsense reasoning tasks, while greatly reducing the need for manual intervention and extensive computational resources.
\end{itemize}

}

\textit{
While outcome supervision does not require process annotation information, making it easier to obtain annotations\ZYQ{ this sentence is confusing: you said "outcome supervision does not require processing annotation" then "easy to obtain annotations?" what do you mean by "it" here?}, process supervision provides evaluations at each step, which aligns with human reasoning logic: if any step contains an error in a reasoning problem, the final result is likely incorrect. 
However, collecting process supervision data is demanding.  However, when questions answering involved multiple reasoning paths, these model-induced methods requires numerous samples to ensure accurate estimations. \ZYQ{wt do you mean by "these"? here, I suppose the these models include both output/process supervised models.}
}

\textit{
To address ths challenge, we propose a novel approach transitioning from outcome to process supervision training, combining the advantages of both methods.
Initially, we generate outcome supervision annotations, determined by whether the final answer is correct, to train an outcome-supervised verification model.
Next, we utilize this trained model to assign step-level scores to unannotated intermediate reasoning steps, reflecting the model's confidence in each step's likelihood of leading to a correct final answer.
By calculating the model's relative confidence variation against a predefined threshold, we develop our \name\ZYQ{necessary to first give the definition of the name before you use it.} labeling strategy and simplify the process of obtaining process annotations.
Furthermore, this process supervision data is utilized to further train the model, resulting in a process-supervised enhanced verification model.
The overall framework of our method is illustrated in~\Cref{fig:orm_process_annotation}.
}
% By calculating the modes' relative confidence vairation agaisng a pre-defined threshold, we devevelop our \name labeeling process and  simplifying the process of obtaining process annotations. 
% Furthermore, this process supervision data is then used to further train the model, resulting in a process-supervised enhanced verification model. 
% The overall framework of our method is illustrated in~\Cref{fig:orm_process_annotation}.

We validate our approach on five datasets, including mathematical reasoning benchmarks and commonsense reasoning tasks.

The extensive experimental results demonstrate that our proposed framework enables efficient and effective automatic process labeling for process supervision without laborious human or compuatational cost.
% Current methods for process annotation primarily rely on either human evaluation~\citep{RewardStep2023,VerifyStep2023}, which can be expensive, especially for complex multi-step reasoning tasks that require skilled annotators, or model-induced process annotation~\citep{MiPS2024,MathShepherd2023}, which esmite the future correctness of the current reasoning step based based on Monte Carlo tree search~\citep{Coulom06,SilverHMGSDSAPL16}   while requires a large number of samples for robust estimation when answering questions involving multiple reasoning paths. 
% Current methods for process annotation primarily rely on either human evaluation~\citep{RewardStep2023,VerifyStep2023}, which can be expensive, especially for complex multi-step reasoning tasks that require skilled annotators, or model-induced process annotation~\citep{MiPS2024,MathShepherd2023}, which introduces a Monte Carlo tree search-based automatic process annotation framework to estimate the future correctness of the current reasoning step. However, these methods still require a large number of samples for robust estimation when answering questions involving multiple reasoning paths.

% Additionally, a well-designed verifier model can also provide valuable feedback to improve the likelihood of an LLM directly outputting the correct answer~\citep{FinegrainedFeedback2023}.
% To address these challenges, previous research has explored various approaches such as through model training or instruction tuning using a substantial amount of chain-of-thought (CoT) reasoning data~\citep{Chung2022,Mukherjee2023,Gunasekar2023,Luo2023}, prompting~\citep{CoT,ComplexityCoT}, and few-shot prompting with intermediate steps augmented demonstration exemplars~\citep{gpt3,CoT,ComplexityCoT} or zero-shot prompting with specific instructions that ask for showing certain intermediate steps~\citep{KojimaGRMI22,Analogical} and  verification~\citep{ProcessFeedback2022, StepAware2023, VerifyStep2023}.


% Large language models (LLMs) have performed remarkably on many reasoning benchmarks~\citep{gpt35turbo,GPT4,mistrallarge,claude3}. These reasoning capabilities of LLMs are typically elicited by prompting techniques~\citep{gpt3}, which can be few-shot prompting with intermediate steps augmented demonstration exemplars~\citep{CoT,ComplexityCoT}, or zero-shot prompting with specific instructions that ask for showing certain intermediate steps~\citep{KojimaGRMI22,Analogical}. The other prevalent strategy for eliciting LLM reasoning is through model training or instruction tuning using a substantial amount of chain-of-thought (CoT) reasoning data~\citep{Chung2022,Mukherjee2023,Gunasekar2023,Luo2023}

% Besides these methods, training a verification model to select candidate responses further improves the accuracy and consistency of the outputs of LLMs. Verification aims to improve reliability by not relying solely on the direct decoding result. 
% Recent research suggests that training a verifier at a step level, rather than relying solely on sparse signals for entire solutions, is more effective~\citep{ProcessFeedback2022, StepAware2023, VerifyStep2023}. Existing verification models can be categorized into two types: Outcome-Supervised Verifier (OSV) and Process-Supervised Verifier (PSV). The OSV is trained on constant labels across all reasoning steps~\citep{CobbeGSM8k2021, YuOVM2023}, while the PSV is provided precise feedback by evaluating each reasoning step individually, resembling human evaluation~\citep{RewardStep2023,VerifyStep2023}. 
% Though PSV offers more detailed feedback and has greater potential for enhancing the generator~\citep{FinegrainedFeedback2023}, building a strong PSV requires extensive process supervision data which require time-consuming annotation cost. 
% Previous work either uses ad-hoc algorithms~\citep{StepAware2023,PaulRefiner2024} or expensive human annotations~\citep{ProcessFeedback2022,VerifyStep2023} to obtain process supervision data, lacking an automatic and generic method for constructing annotations of intermediate solutions.

% Recent approaches~\citep{MathShepherd2023,MiPS2024} propose an automatic process annotation framework based on Monte Carlo Tree Search~\citep{Coulom06,SilverHMGSDSAPL16}. Specifically, for each intermediate solution, the solution is completed with a completor several times through a sample decoding mechanism, and the percentage of the completed solutions being correct is referred to as the correctness of the solution. However, this model-induced labelling strategy still incurs high computational costs, requiring a large number of samples for robust estimation when answering questions involving multiple reasoning paths. 



% To address this challenge, we introduce a novel method for labeling process data by identifying variations in model confidence. 
% We leverage the following key insights: 1. A well-trained OSV model can effectively quantify the probability of the final answer being correct, based on the provided input sequence and question. 2. The relative change in the predicted values shows the model's judgment of whether the current step is correct or not.
% Specifically, we pinpoint relative variations in model confidence to annotate process data. If the relative variation exceeds a threshold, we mark that step as \textit{incorrect}.
% Compared with these model-induced process annotation methods~\cite{MathShepherd2023,MiPS2024}, our approach achieves the same or better results while significantly reducing computational load.
% Extensive experimental results demonstrate the potential of our approach to enhance the precision and scalability of large language models (LLMs) in both mathematical and commonsen reasoning tasks.
% Our proposed framework therefore enables efficient and effective automatic process labeling for process supervision without laborious human effort or computational cost.

% To address this issue, we propose a method to label process data by detecting variations in model confidence. Motivated by relative changes effectively reflecting the model's confidence. Specifically, we detect the relative model confidence variations to annotate the process data \ZJ{Explain more details}. Unlike existing methods that necessitate multiple iterations for labeling, our approach requires only a single generation to label the entire reasoning process, significantly reducing the computational burden while maintain a comparable and even better results in both mathematics and commonsence reasoning datasets. The theoreical guarantee of a verifer can quantifies the probability of the final answer being correct with high probablity and the Extensive experimental results demonstrate the potential of our approach to enhance the precision and scalability of LLMs in various reasoning task demonstrate hthat  our proposed framework enables efficient and effective automatic process labeling for process supervision without laborious human or compuatational cost

% In addition to these methods, training a verification model to select candidate responses further improves the accuracy and consistency of the outputs of LLMs. Verification aims to improve reliability by not relying solely on the greedy decoding result. Previous research has explored verifying intermediate steps rather than the whole solution, as it provides better guidance~\citep{ProcessFeedback2022, StepAware2023, VerifyStep2023}. Existing verification models can be categorized into two types: Outcome  SUpervised Verifier (OSV) and Process Supervised Verifier (PSV). OSV assigns a score to the entire solution~\citep{CobbeGSM8k2021, YuOVM2023}, while PSV provides precise feedback by evaluating reasoning steps individually~\citep{VerifyStep2023, RewardStep2023}. Though PSV offers more detailed feedback and has greater potential for enhancing the generator~\citep{FinegrainedFeedback2023}, building a strong PSV requires extensive process supervision data. Previous work either uses ad-hoc algorithms~\citep{StepAware2023,PaulRefiner2024} or expensive human annotations~\citep{ProcessFeedback2022,VerifyStep2023} to obtain process supervision data, lacking an automatic and generic method for constructing annotations of intermediate solutions.

% Recent approaches~\citep{MathShepherd2023,MiPS2024} propose an automatic process annotation framework based on Monte Carlo Tree Search~\citep{Coulom06,SilverHMGSDSAPL16}. Specifically, for each intermediate solution, the solution is completed with a completor several times through a sample decoding mechanism, and the percentage of the completed solutions being correct is referred to as the correctness of the solution. However, this method incurs high computational costs, requiring a large number of samples for robust estimation $(L \times N)$ when answering questions involving $L$ reasoning paths. \ZJ{Do we want to include the real number they used here to emphasize the computational costs?}

% Math-Shepherd: To determine the label of each reasoning step, we utilize a ‘completer’ to decode N subsequent reasoning processes. We observe that as N increases, so does the quality of automatic annotations. However, this completion process demands a lot of computing resources, potentially imposing a limitation on the usage of our method.


% \ZJ{Computational cost is the only problem they have? What can we offer apart from that?}
% To address this issue, we propose a method to label process data by detecting changes in model confidence. Motivated by relative changes effectively reflecting the model's confidence. Specifically, we incorporate a reliable verifier to detect variations in confidence to annotate the process data \ZJ{Explain more details}. Unlike existing methods that necessitate multiple iterations for labeling, our approach requires only a single generation to label the entire reasoning process, significantly reducing the computational burden $(L \times N)$. This approach enables efficient and effective automatic process labeling for process supervision without laborious human or machine labeling. Extensive experimental results demonstrate the potential of our approach to enhance the precision and scalability of LLMs in various reasoning tasks.





% Large language models (LLMs) have demonstrated remarkable performance on various complicated reasoning benchmarks~\citep{gpt35turbo,GPT4,mistrallarge,claude3}. These reasoning capabilities of LLMs are typically elicited by prompting techniques~\citep{gpt3}, which can be few-shot prompting with intermediate steps augmented demonstration exemplars~\citep{CoT,ComplexityCoT}, or zero-shot prompting with specific instructions that ask for showing certain intermediate steps~\citep{KojimaGRMI22,Analogical}. The other prevalent strategy for eliciting LLM reasoning is through model training or instruction tuning using a substantial amount of chain-of-thought (CoT) reasoning data~\citep{Chung2022,Mukherjee2023,Gunasekar2023,Luo2023}


% Recently, training a verification model in a supervised fashion has demonstrated strong performance in many reasoning tasks. The motivation behind verification is that relying solely on the top-1 result may not always produce reliable outcomes. A verification model can rerank candidate responses, ensuring higher accuracy and consistency in the outputs of LLMs. Early effort~\citep{CobbeGSM8k2021} showed that by simply gathering correct and incorrect solutions to train a binary classification model and using such a model to pick the highest confidence solution generated by the reasoner during inference time, the accuracy can be improved significantly. Recent studies suggest that verifying intermediate steps could offer better guidance than training solely on the whole solutions~\citep{ProcessFeedback2022, StepAware2023, VerifyStep2023}. 

% Existing verification models can be categorized into two types. The Outcome Reward Model (ORM) allocates a score to the entire solution~\citep{CobbeGSM8k2021, YuOVM2023}, while the Process Reward Model (PRM) provides precise feedback by evaluating reasoning steps individually, resembling human judgment~\citep{VerifyStep2023, MathShepherd2023, MiPS2024}. Compared to ORM, PRM provides more detailed feedback, demonstrating the greater potential to enhance generator~\citep{FinegrainedFeedback2023}. To achieve optimal quality, process supervision data is needed for building a strong PRM.  In prior work, process supervision data is either obtained by an ad-hoc algorithm~\citep{StepAware2023,PaulRefiner2024}, or through expensive human annotations~\citep{ProcessFeedback2022,VerifyStep2023}, lacking an automatic and generic way of constructing of annotations of intermediate solutions.

% Recent efforts~\citep{MathShepherd2023,MiPS2024} propose an automatic process annotation framework based on Monte Carlo Tree Search. Specifically, for each intermediate solution, the solution is completed with a completor several times through a sample decoding mechanism, and the percentage of the completed solutions being correct is referred to as the correctness of the solution. Such correctness scores can be used to train a PRM. However, such a method requires extensive computational cost. For instance, when answering a math question involving L reasoning paths, this method requires generating a larger number, N, of samples for robust estimation, resulting in a total cost of (L * N).

% To tackle this problem, we propose to label process data by detecting changes in model confidence. Concretely, our method necessitates a reliable verifier whose relative confidence changes can indicate accuracy or inaccuracy. While their method draws inspiration from Monte Carlo Tree Search, ours operates under the assumption that relative changes effectively reflect the model's confidence. For the same example, when answering a math question involving L reasoning paths, we only need to run one generation to label the entire reasoning process, which is significantly fewer than (L * N). our approach enables a more efficient and effective automatic process labeling for process supervision without extensive human or machine labeling. Extensive experimental results demonstrate the potential of our approach to enhance the precision and scalability of LLMs in various reasoning tasks.

\input{figures/main}   

In summary, our contribution is as follows:
\begin{itemize}
\vspace{-1mm}
\item We introduced A novel method for automatically labeling process data for large language models (LLMs). This method identifies variations in model confidence to annotate the correctness of intermediate reasoning steps, enabling efficient and effective automatic process labeling for process supervision.

\item Comprehensive experiments showcase how  process supervision data from \name improves the performance and scalability of the verification model in mathematical and commonsense reasoning tasks.

\item Our method achieves an automated transition from outcome to process supervision , effectively combining the strengths of both approaches while reducing manual intervention or extensive computational expenses.
\end{itemize}


% In summary, our contribution is threefold:
% \begin{itemize}
% \vspace{-1mm}
% \item By detecting changes in confidence scores, we bridge the gap from outcome-supervision to process-supervision without laborious human labeling.
% \item We provide findings that LLMs without fine-tuning struggle with selection tasks regardless of the prompting strategy, from 7 billion to 70 billion parameter models. We adopt a standard output-supervised fine-tuning method to instill such skills into the 7b parameter LLM.
% \item We introduce a technique to detect calculation errors in mathematical reasoning tasks by monitoring changes in the model's confidence scores during solution steps.
% \end{itemize}


% \textbf{comparison with mips and math shepherd}:Our work and the methods of Math Shepherd and MIPS both delve into the realm of automatically supervising processes induced by models. While Math Shepherd and MIPS utilize model to conduct multiple sampling to estimate the reasoning process, our method labels the process by detecting changes in model confidence.

% Both approaches rely on well-finetuned models. Math Shepherd and MIPS require a proficient completor for completion sampling, whereas our method necessitates a reliable verifier whose relative confidence changes can indicate accuracy or inaccuracy. While their method draws inspiration from Monte Carlo Tree Search, ours operates under the assumption that relative changes effectively reflect the model's confidence.

% We argue that our method boasts a significantly lower computational cost. For instance, when answering a math question involving L reasoning paths, we only need to run one generation to label the entire reasoning process. In contrast, their method requires generating a larger number, N, of samples for a robust estimation, resulting in a total cost of (L * N). We further conduct a fair comparison with their method to glean insights into which approach is more efficient and effective in automatic process labeling.

% In summary, our contribution is threefold:
% \begin{itemize}
% \vspace{-1mm}
%  \item By detecting changes in confidence scores, we bridge the gap from outcome-supervision to process-supervision without laborious human labeling.
%  \item We provide findings that large language models (LLMs) without fine-tuning struggle with selection tasks regardless of the prompting strategy, from 7 billion to 70 billion parameter models. We adopt a standard output-supervised fine-tuning method to instill such skills into the 7b parameter LLM.
%  \item We introduce a technique to detect calculation errors in mathematical reasoning tasks by monitoring changes in the model's confidence scores during solution steps.
%  \end{itemize}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   }                                                                                                                                                                           
